Dynamic Priority Queue: An SDRAM Arbiter With Bounded Access Latencies for Tight WCET Calculation

This report introduces a shared resource arbitration scheme "DPQ - Dynamic Priority Queue" which provides bandwidth guarantees and low worst case latency to each master in an MPSoC. Being a non-trivial candidate for timing analysis, SDRAM has been chosen as a showcase, but the approach is valid for any shared resource arbitration. Due to its significant cost, data rate and physical size advantages, SDRAM is a potential candidate for cost sensitive, safety critical and space conserving systems. The variable access latency is a major drawback of SDRAM that induces largely over estimated Worst Case Execution Time (WCET) bounds of applications. In this report we present the DPQ together with an algorithm to predict the shared SDRAM's worst case latencies. We use the approach to calculate WCET bounds of six hardware tasks executing on an Altera Cyclone III FPGA with shared DDR2 memory. The results show that the DPQ is a fair arbitration scheme and produces low WCET bounds.

==> include/hyphenations.tex <==
\hyphenation{Collision-Chip}
\hyphenation{COLLISION-CHIP}
\hyphenation{comparison}
\hyphenation{complete}
\hyphenation{con-fig-ure}
\hyphenation{DR-FPGA}
\hyphenation{every}
\hyphenation{flexi-bility}
\hyphenation{indicates}
\hyphenation{in-ter-face}
\hyphenation{memory}
\hyphenation{metho-do-logy}
\hyphenation{metho-do-logies}
\hyphenation{module}
\hyphenation{modelling}
\hyphenation{ReChannel}
\hyphenation{RECHANNEL}
\hyphenation{re-con-figur}
\hyphenation{re-con-figur-able}
\hyphenation{re-gis-ter}
\hyphenation{re-gis-tered}
\hyphenation{origin}
\hyphenation{other-wise}
\hyphenation{pro-per-ties}
\hyphenation{se-pa-rat-ing}
\hyphenation{si-mu-lation}
\hyphenation{stra-te-gy}
\hyphenation{systemc}
\hyphenation{SystemC}
\hyphenation{triggered}
\hyphenation{using}


==> include/listings.tex <==
%
% Define usage of listings packge
% includes style definitions for used languages
%
%
\usepackage{color}
\usepackage{listings}

%
% defaults
%
\lstset{
   basicstyle=\small\ttfamily,%
   columns=flexible,%
   tabsize=4,%
   keepspaces,%
   showstringspaces=false,
%   caption=\lstname,
   captionpos=b,
   commentstyle=\textit,%
   keywordstyle=\textbf, %
   stringstyle=\textrm,%
   frame=trbl%
}

\lstdefinestyle{pseudo}%
{    language=C++,%
     morekeywords={START,
	      loop, TRUE, FALSE, times, end, DISPLAY, MOV, LDA, ADI,
              END%
                   },%
     tabsize=4,%
     basicstyle=\ttfamily\small,%
     commentstyle=\rmfamily\textit,%
     keywordstyle=\textbf, %
     stringstyle=\textrm,%
     numberstyle=\tiny,%
     showstringspaces=false
}

\lstdefinestyle{VHDL}%
{    language=VHDL,%
     tabsize=4,%
     basicstyle=\ttfamily\small,%
     commentstyle=\rmfamily\textit,%
     keywordstyle=\textbf, %
     stringstyle=\textrm,%
     numberstyle=\tiny,%
     showstringspaces=false
}

\lstdefinestyle{C++}%
{    language=C++,%
     tabsize=4,%
     basicstyle=\ttfamily\small,%
     commentstyle=\rmfamily\textit,%
     keywordstyle=\textbf, %
     stringstyle=\textrm,%
     numberstyle=\tiny,%
     showstringspaces=false
}

\lstdefinestyle{SystemC}%
{    language=C++,%
     morekeywords={SC_MODULE,SC_CTOR,SC_METHOD,SC_THREAD,SC_CTHREAD,%
                   SC_NS,SC_MS,sc_time,%                 times
                   sc_in,sc_out,sc_fifo_in,sc_fifo_out,% ports
                   sc_signal,sc_fifo,sc_buffer,%         channels
                   sc_int,sc_uint,%                      data types
                   wait,sensitive,sensitive_pos,%        events
                   sc_object,%                           managment
                   sc_find_object%
                   },%
     tabsize=4,%
     basicstyle=\ttfamily\small,%
     commentstyle=\rmfamily\textit,%
     keywordstyle=\color{red}, %
     stringstyle=\textrm,%
     numberstyle=\tiny,%
     showstringspaces=false
}

\lstdefinestyle{ReChannel}%
{    style=SystemC,%
     morekeywords={ rc_control, unload, load, activate, deactivate, takes_time, %rc_control
                    RC_RECONFIGURABLE_MODULE_DERIVED,%  moduls
                    RC_RECONFIGURABLE_CTOR_DERIVED,
                    rc_reconfigurable_module,
                    rc_reconfigurable,
                    rc_portal,%                         portals
                    rc_fifo_in_portal,
                    rc_fifo_out_portal,
                    bind_static,bind_dynamic,%          binding
                    static_port, dynamic_port,
                    rc_portmap, rc_switch_connector,
                    rc_add_portmap
                  }
}

\lstdefinestyle{OSSS}%
{    language=C++,%
     morekeywords={OSSS_TAG,osss_shared,OSSS_SHARED_PC,OSSS_GUARDED,
                   osss_context_base,osss_recon,DURABLE_RECONFIGURABLE,
                   TRANSIENT_RECONFIGURABLE,CONTROLLED_BY,OSSS_DECLARE_TIME,
                   SC_MODULE,SC_CTOR,SC_METHOD,SC_THREAD,SC_CTHREAD,%
                   SC_NS,SC_MS,sc_time,%                 times
                   sc_in,sc_out,sc_fifo_in,sc_fifo_out,% ports
                   sc_signal,sc_fifo,sc_buffer,%         channels
                   sc_int,sc_uint,%                      data types
                   wait,sensitive,sensitive_pos%         events
                   },%
     tabsize=4,%
     basicstyle=\ttfamily\small,%
     commentstyle=\rmfamily\textit,%
     keywordstyle=\color{red}, %
     stringstyle=\textrm,%
     numberstyle=\tiny,%
     showstringspaces=false
}
%
% Fix hyperref toc level
%
\makeatletter\def\toclevel@lstlisting{1}\makeatother

%
% EOF
% vim:set ft=tex tw=75 sts=2 ts=2 sw=2 ai et:
%


==> include/mathops.tex <==
% -----------------------------------------------------------------------
% common sets
% -----------------------------------------------------------------------
\newcommand{\B}{\ensuremath{\mathbb{B}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\Aff}{\ensuremath{\R^3}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}


% -----------------------------------------------------------------------
% common ops
% -----------------------------------------------------------------------
\DeclareMathOperator{\sgn}{sign}
\DeclareMathOperator{\dt}{DT}
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\spos}{sp}
\DeclareMathOperator{\sabs}{sa}
\DeclareMathOperator{\err}{err}
\newcommand{\er}[1]{\err_{#1}}

%  vectors
\newcommand{\vc}[1]{\ensuremath{\mathbf{#1}}}
% matrices
\newcommand{\mat}[1]{\vc{#1}}

% -----------------------------------------------------------------------
% limits of integrals, sums and products above/below symbol
% -----------------------------------------------------------------------
\newcommand{\I}{\int\limits}
\newcommand{\Sum}{\sum\limits}
\newcommand{\Prod}{\prod\limits}



==> include/shortcuts.tex <==
%
% WORKAROUND, damit lstlistoflistings funktioniert:
% Quelle: http://www.komascript.de/node/477
%
\makeatletter
\@ifundefined{float@listhead}{}{%
    \renewcommand*{\lstlistoflistings}{%
        \begingroup
    	    \if@twocolumn
                \@restonecoltrue\onecolumn
            \else
                \@restonecolfalse
            \fi
            \float@listhead{\lstlistlistingname}%
            \setlength{\parskip}{\z@}%
            \setlength{\parindent}{\z@}%
            \setlength{\parfillskip}{\z@ \@plus 1fil}%
            \@starttoc{lol}%
            \if@restonecol\twocolumn\fi
        \endgroup
    }%
}
\makeatother


% for development purposes
\usepackage{ifthen}
\usepackage{calc}

\newboolean{debug}

\newcommand{\red}{\color{red}}
\newcommand{\todo}[1]{ \textit{\textbf{\textcolor{red}{TODO: #1}} }}
\newcommand{\TODO}[1]{ \todo{#1}}
\newcommand{\rema}[2]{ \todo{#1}\textcolor{green}{ #2} }
%\newcommand{\rema}[2]{ { #2} }

%nice to have
%\newcommand{\nth}[1]{}
\newcommand{\nth}[1]{ \textit{\textbf{\textcolor{red}{nice to have: #1}} }}
%\newcommand{\todo}[1]{  }


% beautiful name for libraries
%\newcommand{\ncname}[1]{#1}
\newcommand{\ncname}[1]{\texorpdfstring{\textsc{#1}}{#1}}

%simpler referenzes
%\newcommand{\refSec}[1]{Section ~{\ref{#1}}}
%\newcommand{\refLst}[1]{Listing~{\ref{#1}}}
%\newcommand{\refFig}[1]{Figure ~{\ref{#1}}}
%\newcommand{\refEq}[1]{Equation ~{\ref{#1}}}

%\newcommand{\refSec}[1]{Sec.~{\nameref{#1}}}
%\newcommand{\refSec}[1]{\ifthenelse{\boolean{debug}}{Sec.~$#1$~{\ref{#1}},)}{Sec.~{\ref{#1}}}}
%\newcommand{\refname}[1]{{\em \nameref{#1}}}
\newcommand{\refSecName}[1]{Subsection~{{\em \nameref{#1}}}}
\newcommand{\refSec}[1]{Sec.~{\ref{#1}}}
%\newcommand{\refLst}[1]{\ifthenelse{\boolean{debug}}{Listing~$#1${\ref{#1}}}{Listing~{\ref{#1}}}}
\newcommand{\refLst}[1]{Listing~{\ref{#1}}}
\newcommand{\refFig}[1]{Fig.~{\ref{#1}}}
\newcommand{\refEq}[1]{Eq.~{\ref{#1}}}
%\newcommand{\refEq}[1]{Equation~{\ref{#1}}}
\newcommand{\refTbl}[1]{Table~{\ref{#1}}}


\newcommand{\refpage}[1]{(page~{\pageref{#1}})}

\newcommand{\refsecname}[1]{\refSecName{#1}}
\newcommand{\refsec}[1]{\refSec{#1}}
\newcommand{\refObj}[1]{\refSec{#1}}
\newcommand{\refobj}[1]{\refSec{#1}}
\newcommand{\reflst}[1]{\refLst{#1}}
\newcommand{\reffig}[1]{\refFig{#1}}
\newcommand{\refeq}[1]{\refEq{#1}}
\newcommand{\reftbl}[1]{\refTbl{#1}}

% should be deprecated and moved into \reffig with respect to actual
% language
\newcommand{\Abb}[1]{Abb.~{\ref{#1}}}

% deprecated:
% exists only for compatibility
\newcommand{\Lst}[1]{\refLst{#1}}
\newcommand{\lst}[1]{\reflst{#1}}
\newcommand{\Fig}[1]{\refFig{#1}}
\newcommand{\fig}[1]{\reffig{#1}}

\newcommand{\Sect}[1]{\refSec{#1}}
\newcommand{\sect}[1]{\refsec{#1}}


% deprecated
% better use \verb+...+ instead
\newcommand{\code}{\texttt}
\newcounter{obj}
\newcommand{\objectivref}[2]{
    \refstepcounter{obj}
        {\bf
        \nsublevel{{#2} Objective}
        \label{#1}
    }
}

\newenvironment{objective}{
     \bf
        \vspace{1ex}
    \begin{minipage}{\textwidth}
    \begin{center}
}{
  \end{center} 
    \end{minipage}
}

% upright column entries
% as an evironment
\newenvironment{upcolumn}[1]{\begin{turn}{90}\begin{minipage}{#1}
}{\end{minipage}
\end{turn}
}
%and as command
\newlength{\COLWIDTH}
\newcommand{\upcol}[1]{
    \settowidth{\COLWIDTH}{\begin{tabular}{c} #1 \end{tabular}}
            % use of tabular is a work-around here to allow line-breaks
            % could be more beautiful, but it works and is better than
            % using the environment, anyways...
    \begin{upcolumn}{\COLWIDTH}
        #1
    \end{upcolumn}
}

% minipage mit angepasstergroesse
\newcommand{\flexpage}[1]{
    \settowidth{\COLWIDTH}{\begin{tabular}{c} #1 \end{tabular}}
            % use of tabular is a work-around here to allow line-breaks
            % could be more beautiful, but it works and is better than
            % using the environment, anyways...
    \begin{minipage}{\COLWIDTH}
        #1
    \end{minipage}
}

% for convenience

\newcommand{\bit}[1]{\texorpdfstring{$#1$\hbox{-}bit}{#1-bit}}
\newcommand{\dop}[1]{\texorpdfstring{$#1$\hbox{-}DOP}{#1-DOP}}
\newcommand{\dops}[1]{\texorpdfstring{$#1$\hbox{-}DOPs}{#1-DOPs}}
\newcommand{\kdop}{\dop{k}\xspace}
\newcommand{\kdops}{\dops{k}\xspace}


%\newcommand{\eg}{e\hbox{\.}g\hbox{\.}}
\newcommand{\Eg}{E.g.,\ }
\newcommand{\eg}{e.g.,\ }
\newcommand{\ie}{i.e.,\ }

% can use \ncname directly in code if want to
\newcommand{\rechannel}{\ncname{ReChannel}}
\newcommand{\uniware}{\ncname{UniWaRe}}
\newcommand{\collisionchip}{\ncname{CollisionChip}}
\newcommand{\vhdl}{\ncname{VHDL}}
\newcommand{\verilog}{\ncname{Verilog}}
\newcommand{\matlab}{\ncname{Matlab}}
\newcommand{\SystemC}{\ncname{SystemC}}
\newcommand{\systemc}{\ncname{SystemC}}
\newcommand{\oxl}{\ncname{OCAPI-XL}}
\newcommand{\jhdl}{\ncname{JHDL}}


\newcounter{depth}
\newcommand{\miniparagraph}[1]{ {\em #1}}
\newcommand{\miniminiparagraph}[1]{#1}
\newcommand{\chcklvl}[2] {%
        \ifthenelse{#1=1}{\part{#2}}{}%
        \ifthenelse{#1=2}{\chapter{#2}}{}%
        \ifthenelse{#1=3}{\section{#2}}{}%
        \ifthenelse{#1=4}{\subsection{#2}}{}%
        \ifthenelse{#1=5}{\subsubsection{#2}}{}%
        \ifthenelse{#1=6}{\paragraph{#2}}{}%
        \ifthenelse{#1=7}{\subparagraph{#2}}{}%
        \ifthenelse{#1=8}{\miniparagraph{#2}}{}%
        \ifthenelse{#1=9}{\miniminiparagraph{#2}}{}%
        }
%\newcommand{\chcklvl}[2] {
        %\ifthenelse{#1=0}{\part{#2}}{}
        %\ifthenelse{#1=1}{\chapter{#2}}{}
        %\ifthenelse{#1=2}{\section{#2}}{}
        %\ifthenelse{#1=3}{\subsection{#2}}{}
        %\ifthenelse{#1=4}{\subsubsection{#2}}{}
        %\ifthenelse{#1=5}{\paragraph{#2}}{}
        %\ifthenelse{#1=6}{\subparagraph{#2}}{}
        %\ifthenelse{#1=7}{\miniparagraph{#2}}{}
        %\ifthenelse{#1=8}{\miniminiparagraph{#2}}{}
        %}
\newcommand{\npart}[1]{\setcounter{depth}{1} \chcklvl{\value{depth}}{#1}}
\newcommand{\nchapter}[1]{\setcounter{depth}{2} \chcklvl{\value{depth}}{#1}}
\newcommand{\nsection}[1]{\setcounter{depth}{3} \chcklvl{\value{depth}}{#1}}
\newcommand{\nsubsection}[1]{\setcounter{depth}{4} \chcklvl{\value{depth}}{#1}}
\newcommand{\nsubsubsection}[1]{\setcounter{depth}{5}\chcklvl{\value{depth}}{#1}}
\newcommand{\nparagraph}[1]{\setcounter{depth}{6} \chcklvl{\value{depth}}{#1}}
\newcommand{\nsubparagraph}[1]{\setcounter{depth}{7}\chcklvl{\value{depth}}{#1}}
\newcommand{\nminiparagraph}[1]{\setcounter{depth}{8}\chcklvl{\value{depth}}{#1}}
\newcommand{\level}[1]{
        \chcklvl{\value{depth}}{#1}}
\newcommand{\sublevel}[1]{
        \setcounter{depth}{\value{depth}+1}
        \chcklvl{\value{depth}}{#1}}
\newcounter{dummy}
\newcommand{\nsublevel}[1]{
        \setcounter{dummy}{\value{depth}+1}
        \chcklvl{\value{dummy}}{#1}}
\newcommand{\nsuperlevel}[1]{
        \setcounter{depth}{\value{depth}-1}
        \chcklvl{\value{depth}}{#1}}
\newcommand{\ninclevel}[1]{
        \setcounter{depth}{\value{depth}-#1}}
\newenvironment{lvl}[1]{%
    \setcounter{depth}{\value{depth}+1}%
    \chcklvl{\value{depth}}{#1}%
}{
    \setcounter{depth}{\value{depth}-1}%
}

% delayed 'comma'
\newcommand{\comma}{, }

\newcommand{\shortintertext}{\intertext}

% -----------------------------------------------------------------------
% index helpers
% -----------------------------------------------------------------------
% Command to fix hyperref option hyperindex with bold text
\newcommand{\idxbf}[1]{\textbf{\hyperpage{#1}}}
% command to combine index and output
\newcommand{\txtidx}[2][-]{%
    \ifthenelse{\equal{#1}{-}}%
        {\index{#2}#2}%
        {\index{#1}#2}}

% same as \txtidx, but prints page number in bold (using \idxbf)
\newcommand{\defidx}[2][-]{%
    \ifthenelse{\equal{#1}{-}}%
        {\index{#2|idxbf}#2}%
        {\index{#1|idxbf}#2}}
% -----------------------------------------------------------------------
% Define operator command
%\makeatletter
%\newcommand{\newoperator}[2][]{%
%  \newcommand{\\#2}[2][][]{%
%    \operatorname{#2}%
%        \@ifempty{\#1}{}{^{\#1}}%
%        \@ifempty{\#2}{}{\left( \#2 \right)}%
%  }%
%}
%\makeatother


\endinput
%$Id: shortcuts.tex,v 1.1 2008/08/08 11:49:42 raabe Exp $




